Measuring the Effect of Influential Messages on Varying Personas

Predicting how a user responds to news events enables important applications such as allowing intelligent agents or content producers to estimate the effect on different communities and revise unreleased messages to prevent unexpected bad outcomes such as social conflict and moral injury. We present a new task, Response Forecasting on Personas for News Media, to estimate the response a persona (characterizing an individual or a group) might have upon seeing a news message. Compared to the previous efforts which only predict generic comments to news, the proposed task not only introduces personalization in the modeling but also predicts the sentiment polarity and intensity of each response. This enables more accurate and comprehensive inference on the mental state of the persona. Meanwhile, the generated sentiment dimensions make the evaluation and application more reliable. We create the first benchmark dataset, which consists of 13,357 responses to 3,847 news headlines from Twitter. We further evaluate the SOTA neural language models with our dataset. The empirical results suggest that the included persona attributes are helpful for the performance of all response dimensions. Our analysis shows that the best-performing models are capable of predicting responses that are consistent with the personas, and as a byproduct, the task formulation also enables many interesting applications in the analysis of social network groups and their opinions, such as the discovery of extreme opinion groups.

==> 5.5related.tex <==

\section{Related Work}
\label{sec:experiment}
\subsection{Task Formulation}


as

dialog response generation, we focus on news domain, instead of generating answering user's questions as assistive AI, we focus on analyzing influence on in multiple from events

news comment generation, now personalized

personal emotion pred, we have task & dataset also describing multiple levels  including sentiment, (int), and textual levels; simply predicting the sentiment how different persona would express differently. with an extended definition of persona. In our case, persona attributes apply to a community or individual.
